MUX-PLMs: Data Multiplexing for High-throughput Language Models

The widespread adoption of large language models such as ChatGPT and Bard has led to unprecedented demand for these technologies. The burgeoning cost of inference for ever-increasing model sizes coupled with hardware shortages has limited affordable access and poses a pressing need for efficiency approaches geared towards high throughput and performance. Multi-input multi-output (MIMO) algorithms such as data multiplexing, offer a promising solution with a many-fold increase in throughput by performing inference for multiple inputs at the cost of a single input. Yet these approaches are not currently performant enough to be deployed in modern systems. We change that by developing MUX-PLMs, a class of high throughput pre-trained language models (PLMs) trained with data multiplexing, that can be fine-tuned for any downstream task to yield high-throughput high-performance. Our novel multiplexing and demultiplexing modules proficiently entangle and disentangle inputs, and enable high-performance high throughput \muxplms{} that are competitive with vanilla PLMs while achieving 2x/5x inference speedup with only a $1-4\%$ drop on a broad suite of tasks.

==> 01_title.tex <==
% \title{Pretraining Language Models with Data Multiplexing}
\title{MUX-BERT: Pre-trained Language Models with Data Multiplexing}

\author{
Vishvak Murahari\quad 
Carlos E. Jimenez\quad 
Ameet Deshpande\quad 
Karthik Narasimhan
\AND
\textnormal{Princeton University} \AND
{
\tt \{\href{mailto:murahari@cs.princeton.edu}{murahari},
\href{mailto:carlosej@cs.princeton.edu}{carlosej},
\href{mailto:asd@cs.princeton.edu}{asd},
\href{mailto:karthikn@cs.princeton.edu}{karthikn}\}@cs.princeton.edu
}
}

==> Tables/main_results_table.tex <==
\begin{table*}[t]
\centering
% Resize the table
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{|lccccc|}

\toprule
\textbf{Configuration} & \textbf{GLUE} & \textbf{NER} & \textbf{POS} & \textbf{Throughput} \\
\midrule
DataMUX$_{\textsc{BASE}}$         &      &     &               \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\
DataMUX$_{\textsc{LARGE}}$         &      &     &               \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\
\midrule
BERT$_{\textsc{BASE}}$         &      &     &     &            \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\
BERT$_{\textsc{LARGE}}$  &  &  &   \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\ \midrule
ELECTRA$_{\textsc{BASE}}$         &      &     &               \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\
ELECTRA$_{\textsc{LARGE}}$  &  &  &  \\
\quad $+$ $n=2$  &  &  &  \\
\quad $+$ $n=5$  &  &  &  \\
    \bottomrule
\end{tabular}
\begin{tabular}{@{}cclllll@{}}

\toprule
\multicolumn{1}{l}{\textbf{Architecture}} & \multicolumn{1}{l}{\textbf{Configuration}} & \textbf{Multiplexing} & \textbf{GLUE} & \textbf{NER} & \textbf{POS} & \textbf{Throughput} \\
\midrule
\multirow{14}{*}{\textbf{BERT}}           & \multirow{7}{*}{Base}            & None         &      &     &     &            \\
    &                        & \datamux{} (n=2)  &  &  &  &  \\
    &                        & \datamux{} (n=5)  &  &  &  &  \\
    &                        & \datamux{} (n=10) &  &  &  &  \\
    &                        & \pdatamux{} (n=2)  &  &  &  &  \\
    &                        & \pdatamux{} (n=5)  &  &  &  &  \\
    &                        & \pdatamux{} (n=10) &  &  &  &  \\ \cmidrule(lr){2-7}
    & \multirow{7}{*}{Large}  & None &  &  &  &  \\
    &                        & \datamux{} (n=2)  &  &  &  &  \\
    &                        & \datamux{} (n=5)  &  &  &  &  \\
    &                        & \datamux{} (n=10) &  &  &  &  \\
    &                        & \pdatamux{} (n=2)  &  &  &  &  \\
    &                        & \pdatamux{} (n=5)  &  &  &  &  \\
    &                        & \pdatamux{} (n=10) &  &  &  &  \\ \midrule
    \multirow{14}{*}{\textbf{ELECTRA}}           & \multirow{7}{*}{Base}            & None         &      &     &     &            \\
    &                        & \datamux{} (n=2)  &  &  &  &  \\
    &                        & \datamux{} (n=5)  &  &  &  &  \\
    &                        & \datamux{} (n=10) &  &  &  &  \\
    &                        & \pdatamux{} (n=2)  &  &  &  &  \\
    &                        & \pdatamux{} (n=5)  &  &  &  &  \\
    &                        & \pdatamux{} (n=10) &  &  &  &  \\ \cmidrule(lr){2-7}
    & \multirow{7}{*}{Large}  & None &  &  &  &  \\
    &                        & \datamux{} (n=2)  &  &  &  &  \\
    &                        & \datamux{} (n=5)  &  &  &  &  \\
    &                        & \datamux{} (n=10) &  &  &  &  \\
    &                        & \pdatamux{} (n=2)  &  &  &  &  \\
    &                        & \pdatamux{} (n=5)  &  &  &  &  \\
    &                        & \pdatamux{} (n=10) &  &  &  &  \\ 
    \bottomrule
\end{tabular}
% Resize
}
\caption{
Main results table. \ameet[myself]{This table needs an overhaul. Can we show results only for Large if those are the most impressive results? We can potentially add a column for pre-training time as well.}
\ameet[myself]{Potentially collapse the architecture and configuration columns to make the table more compact.}
\ameet[myself]{Is it possible to transpose the table?}
}
\label{tab:main_results_old}
\end{table*}
